The 2dF-SDSS LRG and QSO Survey: QSO clustering and the L-z degeneracy

We combine the QSO samples from the 2dF QSO Redshift Survey (2QZ) and the 2dF-SDSS LRG and QSO Survey (2SLAQ) in order to investigate the clustering of z~1.4 QSOs and measure the correlation function. The clustering signal in z-space, projected along the sky direction, is similar to that previously obtained from 2QZ alone. By fitting the z-space correlation function and lifting the degeneracy between beta and Omega_m_0 by using linear theory predictions, we obtain beta(z=1.4) = 0.60+-0.12 and Omega_m_0=0.25+-0.08, implying a value for the QSO bias, b(z=1.4)=1.5+-0.2. We further find that QSO clustering does not depend strongly on luminosity at fixed redshift. This result is inconsistent with the expectation of simple `high peaks' biasing models where more luminous, rare QSOs are assumed to inhabit higher mass haloes. The data are more consistent with models which predict that QSOs of different luminosities reside in haloes of similar mass. We find that halo mass does not evolve strongly with redshift nor depend on QSO luminosity. We finally investigate how black hole mass correlates with luminosity and redshift and ascertain the relation between Eddington efficiency and black hole mass. Our results suggest that QSOs of different luminosities may contain black holes of similar mass.

==> abstract <==


The 2dF-SDSS LRG and QSO survey: QSO clustering and the L-$z$ degeneracy

J. da Angela (Durham), T. Shanks (Durham), S.M. Croom (AAO), P. Weilbacher (AIP), R.J. Brunner, W.J. Couch, L. Miller, A.D. Myers, R.C. Nichol, K.A. Pimbblet, R. de Propris, G.T. Richards, N.P. Ross, D.P. Schneider, D.A. Wake

17 pages, 16 figures, 3 tables

We combine the QSO samples from the 2dF QSO Redshift Survey (2QZ) and
the 2dF-SDSS LRG and QSO Survey (2SLAQ) in order to investigate the
clustering of z~1.4 QSOs and measure the correlation function. The
clustering signal in z-space, projected along the sky
direction, is similar to that previously obtained from 2QZ alone. By
fitting the z-space correlation function and lifting the degeneracy
between beta and Omega_m_0  by using linear theory predictions, we
obtain beta(z=1.4) = 0.60+-0.12, \Omega_m_0=0.25+-0.08, implying a
value for the QSO bias, b(z=1.4)=1.5+-0.2. We further find that QSO
clustering does not depend strongly on luminosity at fixed redshift.
This result is inconsistent with the expectation of simple `high peaks'
biasing models where more luminous, rare QSOs are assumed to inhabit
higher mass haloes. The data are more  consistent with models which
predict that QSOs of different luminosities reside in haloes of similar
mass. We find that halo mass does not evolve strongly with redshift nor
depend on QSO luminosity.  We finally investigate how black hole mass
correlates with luminosity and redshift and ascertain the relation
between Eddington efficiency and black hole mass. Our results suggest
that QSOs of different luminosities may contain black holes of similar
mass.

